A boundary quotient diagram for right LCM semigroups

We propose a boundary quotient diagram for right LCM semigroups with property (AR) that generalizes the boundary quotient diagram for the $ax+b$-semigroup over the natural numbers. Our approach focuses on two important subsemigroups: the core subsemigroup and the semigroup of core irreducible elements. The diagram is then employed to unify several case studies on KMS-states, and we end with a discussion on $K$-theoretical aspects of the diagram motivated by recent findings for integral dynamics.

==> bib.tex <==

%\begin{bibdiv}
\begin{biblist}

\bib{ABLS}{article}{
author={Afsar, Zahra},
author={Brownlowe, Nathan},
author={Larsen, Nadia S.},
author={Stammeier, Nicolai},
title={Equilibrium states on right LCM semigroup $C^*$-algebras},
note={preprint, \href{https://arxiv.org/abs/1611.01052}{arxiv:1611.01052}},
}

\bib{AD}{article}{%MR919508,
    AUTHOR ={Anantharaman-Delaroche, Claire},
     TITLE = {Syst\`{e}mes dynamiques non commutatifs et moyennabilit\'{e}},
   JOURNAL = {Math. Ann.},
 % FJOURNAL = {Mathematische Annalen},
    VOLUME = {279},
      YEAR = {1987},
    NUMBER = {2},
     PAGES = {297--315},
      ISSN = {0025-5831},
   %  CODEN = {MAANA},
  % MRCLASS = {46L55 (22D25 22D40 43A07 43A35)},
 % MRNUMBER = {919508 (89f:46127)},
%MRREVIEWER = {Elliot C. Gootman},
       DOI = {\href{http://dx.doi.org/10.1007/BF01461725}{10.1007/BF01461725}},
}

\bib{ADR}{book}{%MR1799683,
    AUTHOR = {Anantharaman-Delaroche, Claire},
    AUTHOR = {Renault, Jean},
     TITLE = {Amenable groupoids},
    SERIES = {Monographies de L'Enseignement Math\'{e}matique},% [Monographs of L'Enseignement Math\'ematique]
    VOLUME = {36},
      NOTE = {With a foreword by Georges Skandalis and Appendix B by E. Germain},
 PUBLISHER = {L'Enseignement Math\'{e}matique, Geneva},
      YEAR = {2000},
     PAGES = {196},
      ISBN = {2-940264-01-5},
   %MRCLASS = {22A22 (22D25 43A07 46L05 46L10 46L80)},
  %MRNUMBER = {1799683 (2001m:22005)},
%MRREVIEWER = {Robert S. Doran},
}

\bib{AM}{article}{
author={Albandik, Suliman},
author={Meyer, Ralf},
title={Product systems over Ore monoids},
note={preprint \href{http://arxiv.org/abs/1502.07768}{arxiv:1502.07768}},
}

\bib{AR}{incollection}{%MR1491110,
    AUTHOR = {Arzumanian, Victor},
    AUTHOR = {Renault, Jean},
     TITLE = {Examples of pseudogroups and their C*-algebras},
 BOOKTITLE = {Operator algebras and quantum field theory ({R}ome, 1996)},
     PAGES = {93--104},
 PUBLISHER = {Int. Press, Cambridge, MA},
      YEAR = {1997},
  % MRCLASS = {46L05},
 % MRNUMBER = {1491110 (99a:46101)},
%MRREVIEWER = {Siegfried Echterhoff},
}

\bib{AS}{article}{%MR1258035,
    AUTHOR = {Archbold, Robert J.},
    AUTHOR = {Spielberg, Jack S.},
     TITLE = {Topologically free actions and ideals in discrete C*-dynamical systems},
   JOURNAL = {Proc. Edinburgh Math. Soc. (2)},
 % FJOURNAL = {Proceedings of the Edinburgh Mathematical Society. Series II},
    VOLUME = {37},
      YEAR = {1994},
    NUMBER = {1},
     PAGES = {119--124},
      ISSN = {0013-0915},
%     CODEN = {PRMSA3},
 %  MRCLASS = {46L55},
  %MRNUMBER = {1258035 (94m:46101)},
%MRREVIEWER = {Yasuyuki Kawahigashi},
       DOI = {\href{http://dx.doi.org/10.1017/S0013091500018733}{10.1017/S0013091500018733}},
}

\bib{Bae}{article}{%MR0009955,
    AUTHOR = {Baer, Reinhold},
     TITLE = {Groups without proper isomorphic quotient groups},
   JOURNAL = {Bull. Amer. Math. Soc.},
  %FJOURNAL = {Bulletin of the American Mathematical Society},
    VOLUME = {50},
      YEAR = {1944},
     PAGES = {267--278},
      ISSN = {0002-9904},
  % MRCLASS = {20.0X},
 % MRNUMBER = {0009955 (5,228a)},
%MRREVIEWER = {I. Kaplansky},
}

\bib{barlak}{thesis}{
    AUTHOR = {Barlak, Sel\c{c}uk},
     TITLE = {On the $K$-theory of Crossed Product {$C^*$}-algebras by Actions of $\mathbb Z^n$},
    SCHOOL = {Westf{\"a}lische Wilhelms-Universit{\"a}t M{\"u}nster},
      YEAR = {2014},
}

\bib{barlak15}{article}{
	AUTHOR={Barlak, Sel\c{c}uk},
	TITLE={On the spectral sequence associated with the Baum-Connes Conjecture for $\mathbb Z^n$},
	NOTE={preprint, \href{http://arxiv.org/abs/1504.03298}{arxiv.org:1504.03298}},
	YEAR={2015},
}

\bib{BOS1}{article}{
	AUTHOR={Barlak, Sel\c{c}uk},
	author={Omland, Tron},
	author={Stammeier, Nicolai},
	TITLE={On the K-theory of $C^*$-algebras arising from integral dynamics},
	journal={Ergodic Theory Dynam. Systems},
	NOTE={(published online)},%preprint, \href{http://arxiv.org/abs/1512.04496}{arxiv.org:1512.04496}},
	YEAR={2016},
	DOI={\href{https://doi.org/10.1017/etds.2016.63}{10.1017/etds.2016.63}},
}


\bib{BarSza1}{article}{
author={Barlak, Sel\c{c}uk},
author={Szab\'{o}, G\'{a}bor},
title={Sequentially split $*$-homomorphisms between $C^*$-algebras},
note={preprint, \href{http://arxiv.org/abs/1510.04555}{arxiv:1510.04555}},
%year={2015},
}


\bib{Ber1}{article}{%MR716835,
    AUTHOR = {Berend, Daniel},
     TITLE = {Multi-invariant sets on tori},
   JOURNAL = {Trans. Amer. Math. Soc.},
  %FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {280},
      YEAR = {1983},
    NUMBER = {2},
     PAGES = {509--532},
      ISSN = {0002-9947},
   %  CODEN = {TAMTAM},
   %MRCLASS = {11K06 (11K55 28D10 54A15)},
  %MRNUMBER = {716835 (85b:11064)},
%MRREVIEWER = {G{\'e}rard Rauzy},
       DOI = {\href{http://dx.doi.org/10.2307/1999631}{10.2307/1999631}},
  %     URL = ,
}

\bib{Ber2}{article}{%MR760973,
    AUTHOR = {Berend, Daniel},
     TITLE = {Multi-invariant sets on compact abelian groups},
   JOURNAL = {Trans. Amer. Math. Soc.},
  %FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {286},
      YEAR = {1984},
    NUMBER = {2},
     PAGES = {505--535},
      ISSN = {0002-9947},
   %  CODEN = {TAMTAM},
   %MRCLASS = {22D40 (11J61 11J69)},
  %MRNUMBER = {760973 (86e:22009)},
%MRREVIEWER = {Justin Peters},
       DOI = {\href{http://dx.doi.org/10.2307/1999808}{10.2307/1999808}},
 %      URL = ,
}

\bib{BD}{article}{%MR0365157,
    AUTHOR = {Bunce, John W.},
    AUTHOR = {Deddens, James A.},
     TITLE = {A family of simple C*-algebras related to weighted shift operators},
   JOURNAL = {J. Funct. Anal.},
    VOLUME = {19},
      YEAR = {1975},
     PAGES = {13--24},
  % MRCLASS = {46LXX (47C10)},
 % MRNUMBER = {0365157 (51 \#1410)},
%MRREVIEWER = {R. G. Douglas},
}

\bib{Bla}{book}{%MR2188261,
    AUTHOR = {Blackadar, Bruce},
     TITLE = {Operator Algebras},
    SERIES = {Encyclopaedia of Mathematical Sciences},
    VOLUME = {122},
     % NOTE = {Theory of C*-Algebras and von Neumann Algebras, Operator Algebras and Non-commutative Geometry, III},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin},
      YEAR = {2006},
     PAGES = {xx+517},
      ISBN = {978-3-540-28486-4; 3-540-28486-9},
  % MRCLASS = {46L05 (46L10 46L80)},
 % MRNUMBER = {2188261 (2006k:46082)},
%MRREVIEWER = {Paul Jolissaint},
}

\bib{BRII}{book}{
    AUTHOR = {Bratteli, Ola},
    AUTHOR = {Robinson, Derek W.},
    TITLE = {Operator algebras and quantum statistical mechanics. Equilibrium states. Models in quantum statistical mechanics. 2nd edition},
    SERIES = {Texts and Monographs in Physics},
    VOLUME = {II},
    PUBLISHER = {Springer-Verlag},
    ADDRESS = {Berlin},
    YEAR =   {1997},
}


\bib{Bri1}{article}{%MR2124335,
    AUTHOR = {Brin, Matthew G.},
     TITLE = {On the {Z}appa-{S}z\'ep product},
   JOURNAL = {Comm. Algebra},
  %FJOURNAL = {Communications in Algebra},
    VOLUME = {33},
      YEAR = {2005},
    NUMBER = {2},
     PAGES = {393--424},
      ISSN = {0092-7872},
    % CODEN = {COALDM},
  % MRCLASS = {20N02 (20M99)},
 % MRNUMBER = {2124335},
%MRREVIEWER = {V{\={\i}}tal{\={\i}}{\u\i} M. Usenko},
       DOI = {\href{http://dx.doi.org/10.1081/AGB-200047404}{10.1081/AGB-200047404}},
  %     URL = {http://dx.doi.org/10.1081/AGB-200047404},
}

\bib{BOFS}{article}{
	AUTHOR = {Brown, Jonathan H.},
  AUTHOR = {Orloff Clark, Lisa},
	AUTHOR = {Farthing, Cynthia},
  AUTHOR = {Sims, Aidan},
  TITLE = {Simplicity of algebras associated to \'{e}tale groupoids},
  JOURNAL = {Semigroup Forum},
%  FJOURNAL = {Semigroup Forum},
    VOLUME = {88},
      YEAR = {2014},
    NUMBER = {2},
     PAGES = {433--452},
      ISSN = {0037-1912},
 %  MRCLASS = {Preliminary Data},
%  MRNUMBER = {3189105},
       DOI = {\href{http://dx.doi.org/10.1007/s00233-013-9546-z}{10.1007/s00233-013-9546-z}},
}

\bib{BO}{book}{%MR2391387,
    AUTHOR = {Brown, Nathanial P.},
    AUTHOR = {Ozawa, Narutaka},
     TITLE = {C*-Algebras and Finite-Dimensional Approximations},
    SERIES = {Graduate Studies in Mathematics},
    VOLUME = {88},
 PUBLISHER = {American Mathematical Society},
   ADDRESS = {Providence, RI},
      YEAR = {2008},
     PAGES = {xvi+509},
      ISBN = {978-0-8218-4381-9; 0-8218-4381-8}
  % MRCLASS = {46L05 (43A07 46-02 46L10)},
 % MRNUMBER = {2391387 (2009h:46101)},
%MRREVIEWER = {Mikael R{\o}rdam},
}

\bib{BaHLR}{article}{
AUTHOR = {Brownlowe, Nathan},
author={an Huef, Astrid},
author={Laca, Marcelo},
author={Raeburn, Iain},
     TITLE = {Boundary quotients of the {T}oeplitz algebra of the affine semigroup over the natural numbers},
   JOURNAL = {Ergodic Theory Dynam. Systems},
%  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {32},
      YEAR = {2012},
    NUMBER = {1},
     PAGES = {35--62},
      ISSN = {0143-3857},
   %MRCLASS = {46L55},
  %MRNUMBER = {2873157 (2012j:46101)},
%MRREVIEWER = {Valentin Deaconu},
       DOI = {\href{http://dx.doi.org/10.1017/S0143385710000830}{10.1017/S0143385710000830}},
%       URL = ,
}

\bib{BLS1}{article}{
	AUTHOR={Brownlowe, Nathan},
	AUTHOR={Larsen, Nadia S.},	
	AUTHOR={Stammeier, Nicolai},
	TITLE={On $C^*$-algebras associated to right LCM semigroups},
	JOURNAL = {Trans. Amer. Math. Soc.},
    VOLUME = {369},
    NUMBER = {1},
    PAGES = {31--68},
	YEAR={2017},
	DOI={\href{http://dx.doi.org/10.1090/tran/6638}{10.1090/tran/6638}},
}

\bib{BLS2}{article}{
	AUTHOR={Brownlowe, Nathan},
	AUTHOR={Larsen, Nadia S.},	
	AUTHOR={Stammeier, Nicolai},
	TITLE={$C^*$-algebras of algebraic dynamical systems and right LCM semigroups},
	NOTE={preprint, \href{http://arxiv.org/abs/1503.01599}{arxiv.org:1503.01599}},
}

\bib{BRRW}{article}{%MR3165249,
    AUTHOR = {Brownlowe, Nathan},
    AUTHOR = {Ramagge, Jacqui},
    AUTHOR = {Robertson, David},
    AUTHOR = {Whittaker, Michael F.},
     TITLE = {Zappa-{S}z\'{e}p products of semigroups and their $C^*$-algebras},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {266},
      YEAR = {2014},
    NUMBER = {6},
     PAGES = {3937--3967},
      ISSN = {0022-1236},
  % MRCLASS = {46L05 (20E08)},
 % MRNUMBER = {3165249},
%MRREVIEWER = {C. J. K. Batty},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2013.12.025}{10.1016/j.jfa.2013.12.025}},
 %      URL = {http://dx.doi.org/10.1016/j.jfa.2013.12.025},
}

\bib{BS1}{article}{
author={Brownlowe, Nathan},
author={Stammeier, Nicolai},
 TITLE = {The boundary quotient for algebraic dynamical systems},
   JOURNAL = {J. Math. Anal. Appl.},
 % FJOURNAL = {Journal of Mathematical Analysis and Applications},
    VOLUME = {438},
      YEAR = {2016},
    NUMBER = {2},
     PAGES = {772--789},
  %    ISSN = {0022-247X},
%   MRCLASS = {Preliminary Data},
%  MRNUMBER = {3466063},
       DOI = {\href{http://dx.doi.org/10.1016/j.jmaa.2016.02.015}{10.1016/j.jmaa.2016.02.015}},
   %    URL = {http://dx.doi.org/10.1016/j.jmaa.2016.02.015},
}


\bib{CLSV}{article}{%MR2837016,
    AUTHOR = {Carlsen, Toke Meier},
    AUTHOR = {Larsen, Nadia S.},
    AUTHOR = {Sims, Aidan},
    AUTHOR = {Vittadello, Sean T.},
     TITLE = {Co-universal algebras associated to product systems, and gauge-invariant uniqueness theorems},
   JOURNAL = {Proc. Lond. Math. Soc. (3)},
%  FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
    VOLUME = {103},
      YEAR = {2011},
    NUMBER = {4},
     PAGES = {563--600},
      ISSN = {0024-6115},
%   MRCLASS = {46L05},
%  MRNUMBER = {2837016 (2012h:46085)},
%MRREVIEWER = {Yangping Jing},
       DOI = {\href{http://dx.doi.org/10.1112/plms/pdq028}{10.1112/plms/pdq028}},
}

\bib{CS}{article}{%MR2563500,
    AUTHOR = {Carlsen, Toke Meier},
    AUTHOR = {Silvestrov, Sergei},
     TITLE = {On the {E}xel crossed product of topological covering maps},
   JOURNAL = {Acta Appl. Math.},
%  FJOURNAL = {Acta Applicandae Mathematicae. An International Survey Journal
%              on Applying Mathematics and Mathematical Applications},
    VOLUME = {108},
      YEAR = {2009},
    NUMBER = {3},
     PAGES = {573--583},
      ISSN = {0167-8019},
%     CODEN = {AAMADV},
%   MRCLASS = {46L55 (37B05)},
%  MRNUMBER = {2563500 (2010k:46071)},
%MRREVIEWER = {Masaharu Kusuda},
       DOI = {\href{http://dx.doi.org/10.1007/s10440-008-9372-6}{10.1007/s10440-008-9372-6}},
}

\bib{Car}{article}{%MR2772352,
    AUTHOR = {Carri{\'o}n, Jos{\'e} R.},
     TITLE = {Classification of a class of crossed product C*-algebras associated with residually finite groups},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {260},
      YEAR = {2011},
    NUMBER = {9},
     PAGES = {2815--2825},
      ISSN = {0022-1236},
%     CODEN = {JFUAAW},
%   MRCLASS = {46L55 (20E26 46L80)},
%  MRNUMBER = {2772352 (2012e:46146)},
%MRREVIEWER = {Nadia S. Larsen},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2011.02.002}{10.1016/j.jfa.2011.02.002}},
}

\bib{Cha}{article}{%MR2322545,
    AUTHOR = {Charney, Ruth},
     TITLE = {An introduction to right-angled {A}rtin groups},
   JOURNAL = {Geom. Dedicata},
%  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {125},
      YEAR = {2007},
     PAGES = {141--158},
      ISSN = {0046-5755},
   %  CODEN = {GEMDAT},
%   MRCLASS = {20F36 (20F65)},
%  MRNUMBER = {2322545},
%MRREVIEWER = {Noelle C. Antony},
       DOI = {\href{http://dx.doi.org/10.1007/s10711-007-9148-6}{10.1007/s10711-007-9148-6}},
   %    URL = {http://dx.doi.org/10.1007/s10711-007-9148-6},
}

\bib{CaHR}{article}{
 AUTHOR = {Clark, Lisa Orloff},
  AUTHOR = {an Huef, Astrid},
   AUTHOR = {Raeburn, Iain},
   TITLE = {Phase transition on the Toeplitz algebra of Baumslag-Solitar semigroups},
   journal={to appear in Indiana Univ. Math. J.},
   NOTE = {preprint \href{http://arxiv.org/abs/1503.04873}{arxiv:1503.04873}},
}


\bib{Com}{article}{%MR748991,
    AUTHOR = {Combes, F.},
     TITLE = {Crossed products and {M}orita equivalence},
   JOURNAL = {Proc. London Math. Soc. (3)},
%  FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
    VOLUME = {49},
      YEAR = {1984},
    NUMBER = {2},
     PAGES = {289--306},
      ISSN = {0024-6115},
%     CODEN = {PLMTAL},
%   MRCLASS = {46L55 (46L05)},
%  MRNUMBER = {748991 (86c:46081)},
       DOI = {\href{http://dx.doi.org/10.1112/plms/s3-49.2.289}{10.1112/plms/s3-49.2.289}},
%       URL = ,
}

\bib{connes}{article}{
title={{An analogue of the Thom isomorphism for crossed products by an action of {$\R$}}},
author={Connes, Alain},
year={1981},
journal={Adv. in Math.},
volume={39},
pages={31--55},
}

\bib{con-mar}{article}{
    AUTHOR = {Connes, Alain},
    AUTHOR = {Marcolli, Matilde},
    TITLE = {Quantum statistical mechanics of $\mathbb{Q}$-lattices},
    SERIES ={In Frontiers in Number Theory, Physics, and Geometry},
    VOLUME = {I},
    PUBLISHER = {Springer},
    YEAR ={2006},
    PAGES = {269--349},
}

\bib{Cos}{article}{%MR1830687,
    AUTHOR = {Veloso da Costa, Ant{\'o}nio},
     TITLE = {Graph products of monoids},
   JOURNAL = {Semigroup Forum},
%  FJOURNAL = {Semigroup Forum},
    VOLUME = {63},
      YEAR = {2001},
    NUMBER = {2},
     PAGES = {247--277},
      ISSN = {0037-1912},
 %    CODEN = {SMGFAN},
  % MRCLASS = {20M05 (68R15)},
  %MRNUMBER = {1830687},
%MRREVIEWER = {Kunitaka Shoji},
       DOI = {\href{http://dx.doi.org/10.1007/s002330010075}{10.1007/s002330010075}},
   %    URL = {http://dx.doi.org/10.1007/s002330010075},
}

\bib{CrispLacaT}{article}{%MR1887134,
    AUTHOR = {Crisp, John},
    author={Laca, Marcelo},
     TITLE = {On the {T}oeplitz algebras of right-angled and finite-type {A}rtin groups},
   JOURNAL = {J. Aust. Math. Soc.},
%  FJOURNAL = {Journal of the Australian Mathematical Society},
    VOLUME = {72},
      YEAR = {2002},
    NUMBER = {2},
     PAGES = {223--245},
      ISSN = {1446-7887},
   %MRCLASS = {46L05 (20F36 46L55 47B35 47L30)},
 % MRNUMBER = {1887134},
%MRREVIEWER = {Sriwulan Adji},
       DOI = {\href{http://dx.doi.org/10.1017/S1446788700003876}{10.1017/S1446788700003876}},
    %   URL = {http://dx.doi.org/10.1017/S1446788700003876},
}

\bib{CrispLaca}{article}{
    AUTHOR = {Crisp, John},
    author={Laca, Marcelo},
     TITLE = {Boundary quotients and ideals of {T}oeplitz {$C^*$}-algebras of {A}rtin groups},
   JOURNAL = {J. Funct. Anal.},
 % FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {242},
      YEAR = {2007},
    NUMBER = {1},
     PAGES = {127--156},
      ISSN = {0022-1236},
     %CODEN = {JFUAAW},
  % MRCLASS = {46L55 (06F15 20F60)},
  %MRNUMBER = {2274018 (2007k:46117)},
%MRREVIEWER = {Alain Valette},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2006.08.001}{10.1016/j.jfa.2006.08.001}},
      % URL = ,
}

\bib{Cun}{article}{%MR0467330,
    AUTHOR = {Cuntz, Joachim},
     TITLE = {Simple C*-algebras generated by isometries},
   JOURNAL = {Comm. Math. Phys.},
%  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {57},
      YEAR = {1977},
    NUMBER = {2},
     PAGES = {173--185},
      ISSN = {0010-3616},
%   MRCLASS = {46L05},
%  MRNUMBER = {0467330 (57 \#7189)},
%MRREVIEWER = {E. Stormer},
}

\bib{CuntzQ}{incollection}{
    AUTHOR = {Cuntz, Joachim},
     TITLE = {{$C^*$}-algebras associated with the {$ax+b$}-semigroup over {$\mathbb{N}$}},
 BOOKTITLE = {{$K$}-theory and noncommutative geometry},
    SERIES = {EMS Ser. Congr. Rep.},
     PAGES = {201--215},
 PUBLISHER = {Eur. Math. Soc., Z\"urich},
      YEAR = {2008},
}

\bib{CEL}{article}{
	AUTHOR = {Cuntz, Joachim},
    AUTHOR = {Echterhoff, Siegfried},
    AUTHOR = {Li, Xin},
     TITLE = {On the $K$-theory of the C*-algebra generated by the left regular representation of an Ore semigroup}, %{$K$}
     JOURNAL = {to appear in J. Eur. Math. Soc.}
      YEAR = {2014},
       NOTE = {available as \href{http://arxiv.org/abs/1201.4680}{arxiv:1201.4680}},
}	

\bib{CEL2}{article}{%MR3094498,
AUTHOR = {Cuntz, Joachim},
AUTHOR = {Echterhoff, Siegfried},
AUTHOR = {Li, Xin},
TITLE = {On the $K$-theory of crossed products by automorphic semigroup actions}, %{$K$}
JOURNAL = {Q. J. Math.},
%FJOURNAL = {The Quarterly Journal of Mathematics},
VOLUME = {64},
YEAR = {2013},
NUMBER = {3},
     PAGES = {747--784},
      ISSN = {0033-5606},
   %MRCLASS = {19Dxx},
  %MRNUMBER = {3094498},
       DOI = {\href{http://dx.doi.org/10.1093/qmath/hat021}{10.1093/qmath/hat021}},
}	

\bib{CK}{article}{%MR561974,
    AUTHOR = {Cuntz, Joachim},
    AUTHOR = {Krieger, Wolfgang},
     TITLE = {A class of C*-algebras and topological {M}arkov chains},
   JOURNAL = {Invent. Math.},
  %FJOURNAL = {Inventiones Mathematicae},
    VOLUME = {56},
      YEAR = {1980},
    NUMBER = {3},
     PAGES = {251--268},
      ISSN = {0020-9910},
     %CODEN = {INVMBH},
   %MRCLASS = {46L55 (54H20 58G10)},
  %MRNUMBER = {561974 (82f:46073a)},
%MRREVIEWER = {R. J. Nagel},
       DOI = {\href{http://dx.doi.org/10.1007/BF01390048}{10.1007/BF01390048}},
}

\bib{CL}{incollection}{%MR2732050,
    AUTHOR = {Cuntz, Joachim},
    AUTHOR = {Li, Xin},
     TITLE = {The regular C*-algebra of an integral domain},
 BOOKTITLE = {Quanta of maths},
    SERIES = {Clay Math. Proc.},
    VOLUME = {11},
     PAGES = {149--170},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2010},
  % MRCLASS = {46L55 (11M55 11R04 46L05)},
 % MRNUMBER = {2732050 (2012c:46173)},
%MRREVIEWER = {Bora Yalkinoglu},
}

\bib{CLintegral2}{article}{
    AUTHOR = {Cuntz, Joachim},
    author={Li, Xin},
     TITLE = {{$C^*$}-algebras associated with integral domains and crossed products by actions on adele spaces},
   JOURNAL = {J. Noncommut. Geom.},
 % FJOURNAL = {Journal of Noncommutative Geometry},
    VOLUME = {5},
      YEAR = {2011},
    NUMBER = {1},
     PAGES = {1--37},
      ISSN = {1661-6952},
}

\bib{CuntzVershik}{article}{
		AUTHOR = {Cuntz, Joachim},
		author={Vershik, Anatoly},
     TITLE = {{$C^*$}-algebras associated with endomorphisms and polymorphisms of compact abelian groups},
      YEAR = {2013},
issn={0010-3616},
journal={Comm. Math. Phys.},
volume={321},
number={1},
doi= {\href{http://dx.doi.org/10.1007/s00220-012-1647-0}{10.1007/s00220-012-1647-0}},
publisher={Springer-Verlag},
pages={157-179},
%language={English}
}	

\bib{DE}{book}{%MR2457798,
    AUTHOR = {Deitmar, Anton},
    AUTHOR = {Echterhoff, Siegfried},
     TITLE = {Principles of Harmonic Analysis},
    SERIES = {Universitext},
 PUBLISHER = {Springer, New York},
      YEAR = {2009},
     PAGES = {xvi+333},
      ISBN = {978-0-387-85468-7},
  % MRCLASS = {43-01 (22Dxx 22E30 46J10 46L05)},
 % MRNUMBER = {2457798 (2010g:43001)},
%MRREVIEWER = {Krishnan Parthasarathy},
}

\bib{DFK}{article}{
 	AUTHOR 	= {Davidson, Kenneth R.},
    AUTHOR 	= {Fuller, Adam H.},
    AUTHOR 	= {Kakariadis, Evgenios T.A.},
    TITLE	= {Semicrossed products of operator algebras by semigroups},
    %JOURNAL = {preprint},
    NOTE 	= {preprint \href{http://arxiv.org/abs/1404.1906v1}{arxiv:1404.1906v1}},
}

\bib{Die}{book}{%MR1075995,
    AUTHOR = {Diekert, Volker},
     TITLE = {Combinatorics on traces},
    SERIES = {Lecture Notes in Computer Science},
    VOLUME = {454},
      NOTE = {With a foreword by Wilfried Brauer},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {1990},
     PAGES = {xii+165},
      ISBN = {3-540-53031-2},
   %MRCLASS = {68Q42 (05C85 20M05 68Q10 68R15)},
  %MRNUMBER = {1075995},
%MRREVIEWER = {John Shawe-Taylor},
       DOI = {\href{http://dx.doi.org/10.1007/3-540-53031-2}{10.1007/3-540-53031-2}},
       URL = {http://dx.doi.org/10.1007/3-540-53031-2},
}

\bib{DG}{article}{%MR2055042,
    AUTHOR = {Duncan, Andrew},
    AUTHOR = {Gilman, Robert H.},
     TITLE = {Word hyperbolic semigroups},
   JOURNAL = {Math. Proc. Cambridge Philos. Soc.},
%  FJOURNAL = {Mathematical Proceedings of the Cambridge Philosophical Society},
    VOLUME = {136},
      YEAR = {2004},
    NUMBER = {3},
     PAGES = {513--524},
      ISSN = {0305-0041},
%     CODEN = {MPCPCO},
  % MRCLASS = {20M05 (20M35)},
%  MRNUMBER = {2055042 (2004m:20106)},
%MRREVIEWER = {P. M. Higgins},
       DOI = {\href{http://dx.doi.org/10.1017/S0305004103007497}{10.1017/S0305004103007497}},
%       URL = ,
}

\bib{dJST}{article}{%MR2913686,
    AUTHOR = {de Jeu, Marcel},
    AUTHOR = {Svensson, Christian},
    AUTHOR = {Tomiyama, Jun},
     TITLE = {On the {B}anach {$\ast$}-algebra crossed product associated with a topological dynamical system},
   JOURNAL = {J. Funct. Anal.},
 % FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {262},
      YEAR = {2012},
    NUMBER = {11},
     PAGES = {4746--4765},
      ISSN = {0022-1236},
   %  CODEN = {JFUAAW},
  % MRCLASS = {46L55 (46H99 54H20)},
 % MRNUMBER = {2913686},
%MRREVIEWER = {Claire Anantharaman-Delaroche},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2012.03.013}{10.1016/j.jfa.2012.03.013}},
       %URL = ,
}

\bib{dlH}{book}{%MR1786869,
    AUTHOR = {de la Harpe, Pierre},
     TITLE = {Topics in Geometric Group Theory},
    SERIES = {Chicago Lectures in Mathematics},
 PUBLISHER = {University of Chicago Press, Chicago, IL},
      YEAR = {2000},
     PAGES = {vi+310},
      ISBN = {0-226-31719-6; 0-226-31721-8},
  % MRCLASS = {20F65 (20F69 57M07)},
 % MRNUMBER = {1786869 (2001i:20081)},
%MRREVIEWER = {Lee Mosher},
}

\bib{ELR}{article}{%MR3505132,
    AUTHOR = {Eilers, S{\o}ren},
    author={Li, Xin},
    author={Ruiz, Efren},
     TITLE = {The isomorphism problem for semigroup {$C\sp *$}-algebras of right-angled {A}rtin monoids},
   JOURNAL = {Doc. Math.},
  %FJOURNAL = {Documenta Mathematica},
    VOLUME = {21},
      YEAR = {2016},
     PAGES = {309--343},
      ISSN = {1431-0635},
   %MRCLASS = {46L05 (20M05 46L35)},
  %MRNUMBER = {3505132},
  NOTE={\href{http://www.math.uiuc.edu/documenta/vol-21/11.html}{electronic version}},
}

\bib{EF}{article}{%MR2586349,
    AUTHOR = {Einsiedler, Manfred},
    AUTHOR = {Fish, Alexander},
     TITLE = {Rigidity of measures invariant under the action of a multiplicative semigroup of polynomial growth on $\IT$},
   JOURNAL = {Ergodic Theory Dynam. Systems},
 % FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {30},
      YEAR = {2010},
    NUMBER = {1},
     PAGES = {151--157},
      ISSN = {0143-3857},
 %  MRCLASS = {37A10 (28D10 37A25)},
 % MRNUMBER = {2586349 (2011a:37005)},
%MRREVIEWER = {A. I. Danilenko},
       DOI = {\href{http://dx.doi.org/10.1017/S014338570800103X}{10.1017/S014338570800103X}},
}

\bib{EK}{article}{%MR2191228,
    AUTHOR = {Einsiedler, Manfred},
    AUTHOR = {Katok, Anatole},
     TITLE = {Rigidity of measures---the high entropy case and non-commuting foliations},
 %     NOTE = {Probability in mathematics},
   JOURNAL = {Israel J. Math.},
%  FJOURNAL = {Israel Journal of Mathematics},
    VOLUME = {148},
      YEAR = {2005},
     PAGES = {169--238},
      ISSN = {0021-2172},
 %    CODEN = {ISJMAP},
 %  MRCLASS = {37C85 (37A15 37C40 37D30)},
 % MRNUMBER = {2191228 (2007d:37034)},
%MRREVIEWER = {S. G. Dani},
       DOI = {\href{http://dx.doi.org/10.1007/BF02775436}{10.1007/BF02775436}},
%       URL = ,
}

\bib{ER2}{article}{%MR2162134,
    AUTHOR = {Endimioni, G{\'e}rard},
    AUTHOR = {Robinson, Derek J. S.},
     TITLE = {On co-{H}opfian groups},
   JOURNAL = {Publ. Math. Debrecen},
 % FJOURNAL = {Publicationes Mathematicae Debrecen},
    VOLUME = {67},
      YEAR = {2005},
    NUMBER = {3-4},
     PAGES = {423--436},
      ISSN = {0033-3883},
   %  CODEN = {PUMAAR},
  % MRCLASS = {20F99},
 % MRNUMBER = {2162134 (2006e:20082)},
%MRREVIEWER = {Javier Otal},
}

\bib{Evans}{article}{
AUTHOR = {Evans, D. Gwion},
     TITLE = {On the {$K$}-theory of higher rank graph {$C\sp *$}-algebras},
   JOURNAL = {New York J. Math.},
 % FJOURNAL = {New York Journal of Mathematics},
    VOLUME = {14},
      YEAR = {2008},
     PAGES = {1--31},
      ISSN = {1076-9803},
 %  MRCLASS = {46L80 (19K14 46L35 46M18)},
  %MRNUMBER = {2383584 (2009e:46065)},
%MRREVIEWER = {Benton L. Duncan},
       URL = {\href{http://nyjm.albany.edu:8000/j/2008/14_1.html}{nyjm:8000/j/2008/14_1}},
}

\bib{Ex}{article}{
	title={The soft torus and applications to almost commuting matrices},
	author={Exel, R.},
	year={1993},
	journal={Pacific J. Math.},
	volume={160},
	number={2},
	pages={207--217}
}

\bib{Exe1}{article}{%MR2032486,
    AUTHOR = {Exel, Ruy},
     TITLE = {A new look at the crossed-product of a C*-algebra by an endomorphism},
   JOURNAL = {Ergodic Theory Dynam. Systems},
 % FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {23},
      YEAR = {2003},
    NUMBER = {6},
     PAGES = {1733--1750},
      ISSN = {0143-3857},
  % MRCLASS = {46L55 (37B10)},
 % MRNUMBER = {2032486 (2004k:46119)},
%MRREVIEWER = {Sriwulan Adji},
       DOI = {\href{http://dx.doi.org/10.1017/S0143385702001797}{10.1017/S0143385702001797}},
}

\bib{Exe2}{article}{%MR1966826,
    AUTHOR = {Exel, Ruy},
     TITLE = {Crossed-products by finite index endomorphisms and {KMS} states},
   JOURNAL = {J. Funct. Anal.},
 % FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {199},
      YEAR = {2003},
    NUMBER = {1},
     PAGES = {153--188},
      ISSN = {0022-1236},
   %  CODEN = {JFUAAW},
  % MRCLASS = {46L55 (46L30)},
 % MRNUMBER = {1966826 (2004b:46094)},
%MRREVIEWER = {Masaharu Kusuda},
       DOI = {\href{http://dx.doi.org/10.1016/S0022-1236(02)00023-X}{10.1016/S0022-1236(02)00023-X}},
}

\bib{EaHR}{article}{%MR2985865,
    AUTHOR = {Exel, Ruy},
    AUTHOR = {an Huef, Astrid},
    AUTHOR = {Raeburn, Iain},
     TITLE = {Purely infinite simple {$C^*$}-algebras associated to integer dilation matrices},
   JOURNAL = {Indiana Univ. Math. J.},
 % FJOURNAL = {Indiana University Mathematics Journal},
    VOLUME = {60},
      YEAR = {2011},
    NUMBER = {3},
     PAGES = {1033--1058},
      ISSN = {0022-2518},
%     CODEN = {IUMJAB},
 %  MRCLASS = {46L05 (46L55)},
  %MRNUMBER = {2985865},
%MRREVIEWER = {Xin Li},
       DOI = {\href{http://dx.doi.org/10.1512/iumj.2011.60.4331}{10.1512/iumj.2011.60.4331}},
       %URL = ,
}

\bib{EP}{article}{
    AUTHOR = {Exel, Ruy},
    AUTHOR = {Pardo, Enrique},
     TITLE = {The tight groupoid of an inverse semigroup},
DOI = {\href{http://arxiv.org/abs/1408.5278v2}{arxiv:1408.5278v2}},
}

\bib{ER}{article}{%MR2371594,
    AUTHOR = {Exel, Ruy},
    AUTHOR = {Renault, Jean},
     TITLE = {Semigroups of local homeomorphisms and interaction groups},
   JOURNAL = {Ergodic Theory Dynam. Systems},
 % FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {27},
      YEAR = {2007},
    NUMBER = {6},
     PAGES = {1737--1771},
      ISSN = {0143-3857},
  % MRCLASS = {46L55 (37B05 46L05)},
 % MRNUMBER = {2371594 (2009k:46124)},
       DOI = {\href{http://dx.doi.org/10.1017/S0143385707000193}{10.1017/S0143385707000193}},
}	

\bib{EV}{article}{%MR2195591,
    AUTHOR = {Exel, Ruy},
    AUTHOR = {Vershik, Anatoly},
     TITLE = {C*-algebras of irreversible dynamical systems},
   JOURNAL = {Canad. J. Math.},
%  FJOURNAL = {Canadian Journal of Mathematics. Journal Canadien de
%              Math\'ematiques},
    VOLUME = {58},
      YEAR = {2006},
    NUMBER = {1},
     PAGES = {39--63},
      ISSN = {0008-414X},
%     CODEN = {CJMAAB},
%   MRCLASS = {46L55 (37A55 46L05)},
%  MRNUMBER = {2195591 (2007d:46058)},
%MRREVIEWER = {Fr{\'e}d{\'e}ric Latr{\'e}moli{\`e}re},
       DOI = {\href{http://dx.doi.org/10.4153/CJM-2006-003-x}{10.4153/CJM-2006-003-x}},
}


\bib{FPW}{article}{%MR3085824,
    AUTHOR = {Farthing, Cynthia},
    AUTHOR = {Patani, Nura},
    AUTHOR = {Willis, Paulette N.},
     TITLE = {The crossed-product structure of C*-algebras arising from topological dynamical systems},
   JOURNAL = {J. Operator Theory},
  %FJOURNAL = {Journal of Operator Theory},
    VOLUME = {70},
      YEAR = {2013},
    NUMBER = {1},
     PAGES = {191--210},
      ISSN = {0379-4024},
   %MRCLASS = {46L55 (37A55)},
  %MRNUMBER = {3085824},
       DOI = {\href{http://dx.doi.org/10.7900/jot.2011may31.1924}{10.7900/jot.2011may31.1924}},
}

\bib{FK}{article}{%MR2551120,
    AUTHOR = {Fountain, John},
    author={Kambites, Mark},
     TITLE = {Graph products of right cancellative monoids},
   JOURNAL = {J. Aust. Math. Soc.},
%  FJOURNAL = {Journal of the Australian Mathematical Society},
    VOLUME = {87},
      YEAR = {2009},
    NUMBER = {2},
     PAGES = {227--252},
      ISSN = {1446-7887},
%   MRCLASS = {20M10 (20M12 20M18)},
%  MRNUMBER = {2551120},
%MRREVIEWER = {V{\'a}clav Koubek},
       DOI = {\href{http://dx.doi.org/10.1017/S144678870900010X}{10.1017/S144678870900010X}},
    %   URL = {http://dx.doi.org/10.1017/S144678870900010X},
}

\bib{Fow1}{article}{%MR1715181,
    AUTHOR = {Fowler, Neal J.},
    TITLE = {Compactly-aligned discrete product systems, and generalization of $\CO_{\infty}$},
   JOURNAL = {Internat. J. Math.},
  %FJOURNAL = {International Journal of Mathematics},
    VOLUME = {10},
      YEAR = {1999},
    NUMBER = {6},
     PAGES = {721--738},
      ISSN = {0129-167X},
  % MRCLASS = {46L05},
 % MRNUMBER = {1715181 (2002f:46104)},
       DOI = {\href{http://dx.doi.org/10.1142/S0129167X99000306}{10.1142/S0129167X99000306}},
}

\bib{Fow2}{article}{%MR1907896,
    AUTHOR = {Fowler, Neal J.},
     TITLE = {Discrete product systems of {H}ilbert bimodules},
   JOURNAL = {Pacific J. Math.},
 % FJOURNAL = {Pacific Journal of Mathematics},
    VOLUME = {204},
      YEAR = {2002},
    NUMBER = {2},
     PAGES = {335--375},
      ISSN = {0030-8730},
%     CODEN = {PJMAAI},
%   MRCLASS = {46L08},
%  MRNUMBER = {1907896 (2003g:46070)},
%MRREVIEWER = {Arup Kumar Pal},
       DOI = {\href{http://dx.doi.org/10.2140/pjm.2002.204.335}{10.2140/pjm.2002.204.335}},
}

\bib{FS}{article}{
AUTHOR = {Fowler, Neal J.},
author={Sims, Aidan},
     TITLE = {Product systems over right-angled {A}rtin semigroups},
   JOURNAL = {Trans. Amer. Math. Soc.},
  %FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {354},
      YEAR = {2002},
    NUMBER = {4},
     PAGES = {1487--1509 (electronic)},
      ISSN = {0002-9947},
     %CODEN = {TAMTAM},
   %MRCLASS = {18D10 (18B40 20F36 46L06)},
 % MRNUMBER = {1873016 (2002j:18006)},
%MRREVIEWER = {V{\'a}clav Koubek},
     URL = {\href{http://dx.doi.org/10.1090/S0002-9947-01-02911-7}{$10.1090/S0002-9947-01-02911-7$}},
}

\bib{Fur}{article}{%MR0213508,
    AUTHOR = {Furstenberg, Hillel},
     TITLE = {Disjointness in ergodic theory, minimal sets, and a problem in {D}iophantine approximation},
   JOURNAL = {Math. Systems Theory},
  %FJOURNAL = {Mathematical Systems Theory. An International Journal on
%              Mathematical Computing Theory},
    VOLUME = {1},
      YEAR = {1967},
     PAGES = {1--49},
      ISSN = {0025-5661},
   %MRCLASS = {28.70 (10.00)},
 % MRNUMBER = {0213508 (35 \#4369)},
%MRREVIEWER = {W. Parry}
}


\bib{Ga}{book} {%MR0107648,
    AUTHOR = {Gantmacher, F. R.},
     TITLE = {Applications of the theory of matrices},
    SERIES = {Translated by J. L. Brenner, with the assistance of D. W. Bushaw and S. Evanusa},
 PUBLISHER = {Interscience Publishers, Inc., New York},
      YEAR = {1959},
     PAGES = {ix+317}
  % MRCLASS = {15.00 (65.00)},
 % MRNUMBER = {0107648 (21 \#6372b)},
}

\bib{GG}{incollection}{%MR2962880,
    AUTHOR = {Goldsmith, Brendan},
    AUTHOR = {Gong, Ketao},
     TITLE = {A note on {H}opfian and co-{H}opfian abelian groups},
 BOOKTITLE = {Groups and Model Theory},
    SERIES = {Contemp. Math.},
    VOLUME = {576},
     PAGES = {129--136},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2012},
  % MRCLASS = {20K30 (20K21)},
 % MRNUMBER = {2962880},
%MRREVIEWER = {Simion Sorin P. Breaz},
       DOI = {\href{http://dx.doi.org/10.1090/conm/576/11356}{10.1090/conm/576/11356}},
}

\bib{Gl}{article}{
	AUTHOR = {Glimm, James G.},
	TITLE = {On a certain class of operator algebras},
	JOURNAL = {Trans. Amer. Math. Soc.},
	VOLUME = {95},
	YEAR = {1960},
	PAGES = {318--340}
}

\bib{Gre}{thesis}{
    AUTHOR = {Green, Elisabeth R.},
     TITLE = {Graph products of groups},
    SCHOOL = {University of Leeds},
      YEAR = {1990},
}

\bib{Hed}{article}{%MR0259881,
    AUTHOR = {Hedlund, Gustav A.},
     TITLE = {Endomorphisms and automorphisms of the shift dynamical system},
   JOURNAL = {Math. Systems Theory},
%  FJOURNAL = {Mathematical Systems Theory. An International Journal on Mathematical Computing Theory},
    VOLUME = {3},
      YEAR = {1969},
     PAGES = {320--375},
      ISSN = {0025-5661},
  % MRCLASS = {54.82},
 % MRNUMBER = {0259881 (41 \#4510)},
%MRREVIEWER = {W. R. Utz},
}

\bib{hr}{book}{ %MR0156915
   author={Hewitt, Edwin},
   author={Ross, Kenneth A.},
   title={Abstract harmonic analysis. Vol. I: Structure of topological
   groups. Integration theory, group representations},
   series={Die Grundlehren der mathematischen Wissenschaften, Bd. 115},
   publisher={Academic Press, Inc., Publishers, New York; Springer-Verlag,
   Berlin-G\"ottingen-Heidelberg},
   date={1963},
   pages={viii+519},
   review={\MR{0156915 (28 \#158)}},
}

\bib{Hir}{article} {%MR1896827,
    AUTHOR = {Hirshberg, Ilan},
     TITLE = {On $C^*$-algebras associated to certain endomorphisms of discrete groups},
   JOURNAL = {New York J. Math.},
  %FJOURNAL = {New York Journal of Mathematics},
    VOLUME = {8},
      YEAR = {2002},
     PAGES = {99--109 (electronic)},
      ISSN = {1076-9803},
  % MRCLASS = {46L55},
 % MRNUMBER = {1896827 (2003d:46090)},
%MRREVIEWER = {Sriwulan Adji},
       NOTE = {\href{http://nyjm.albany.edu:8000/j/2002/8_99.html}{$nyjm.albany.edu:8000/j/2002/8_99$}},
}

\bib{HLS}{article}{
AUTHOR = {Hong, Jeong Hee},
AUTHOR = {Larsen, Nadia S.},
AUTHOR = {Szyma\'{n}ski, Wojciech},
TITLE  = {KMS states on Nica-Toeplitz algebras of product systems},
journal = {Internat. J. Math.},
volume = {23},
number = {12},
pages = {1250123},
year = {2012},
doi = {\href{http://www.worldscientific.com/doi/abs/10.1142/S0129167X12501236}{10.1142/S0129167X12501236}},
%eprint = {http://www.worldscientific.com/doi/pdf/10.1142/S0129167X12501236}
}

\bib{aHLRS}{article}{%MR3315580,
    AUTHOR = {an Huef, Astrid},
    author={Laca, Marcelo},
    author={Raeburn, Iain},
    author={Sims, Aidan},
     TITLE = {K{MS} states on the {$C\sp *$}-algebra of a higher-rank graph and periodicity in the path space},
   JOURNAL = {J. Funct. Anal.},
 % FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {268},
      YEAR = {2015},
    NUMBER = {7},
     PAGES = {1840--1875},
      ISSN = {0022-1236},
  % MRCLASS = {46L30 (46L55)},
 % MRNUMBER = {3315580},
%MRREVIEWER = {Camillo Trapani},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2014.12.006}{10.1016/j.jfa.2014.12.006}},
  %     URL = {http://dx.doi.org/10.1016/j.jfa.2014.12.006},
}

\bib{JT}{book} {%MR1124848,
    AUTHOR = {Jensen, Kjeld Knudsen},
    AUTHOR = {Thomsen, Klaus},
     TITLE = {Elements of {$KK$}-Theory},
    SERIES = {Mathematics: Theory \& Applications},
 PUBLISHER = {Birkh\"auser Boston Inc.},
   ADDRESS = {Boston, MA},
      YEAR = {1991},
     PAGES = {viii+202},
      ISBN = {0-8176-3496-7},
  % MRCLASS = {19K35 (46L80)},
 % MRNUMBER = {1124848 (94b:19008)},
%MRREVIEWER = {Jeffrey Fox},
       DOI = {\href{http://dx.doi.org/10.1007/978-1-4612-0449-7}{10.1007/978-1-4612-0449-7}},
}

\bib{KOQ}{article}{ %MR3300223
   author={Kaliszewski, S.},
   author={Omland, Tron},
   author={Quigg, John},
   title={Cuntz-Li algebras from $a$-adic numbers},
   journal={Rev. Roumaine Math. Pures Appl.},
   volume={59},
   date={2014},
   number={3},
   pages={331--370},
   issn={0035-3965},
   review={\MR{3300223}},
}

\bib{kasparov}{article}{
author={Kasparov, Gennadi},
title={{Equivariant {$KK$}-theory and the Novikov conjecture}},
volume={91},
journal={Invent. Math.},
year={1988},
pages={147--201},
}

\bib{KatsuraI}{article} {%MR2067120,
    AUTHOR = {Katsura, Takeshi},
     TITLE = {A class of C*-algebras generalizing both graph algebras and homeomorphism C*-algebras. {I}. {F}undamental results},
   JOURNAL = {Trans. Amer. Math. Soc.},
  %FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {356},
      YEAR = {2004},
    NUMBER = {11},
     PAGES = {4287--4322 (electronic)},
      ISSN = {0002-9947},
    % CODEN = {TAMTAM},
   %MRCLASS = {46L05 (37B99 46L55 46L80)},
 %MRNUMBER = {2067120 (2005b:46119)},
%MRREVIEWER = {Valentin Deaconu},
       DOI = {\href{http://dx.doi.org/10.1090/S0002-9947-04-03636-0}{10.1090/S0002-9947-04-03636-0}},
}

\bib{KatsuraIV}{article}{
    AUTHOR = {Katsura, Takeshi},
     TITLE = {A class of {$C^*$}-algebras generalizing both graph algebras and homeomorphism {$C^*$}-algebras. {IV}. {P}ure infiniteness},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {254},
      YEAR = {2008},
    NUMBER = {5},
     PAGES = {1161--1187},
      ISSN = {0022-1236},
 %    CODEN = {JFUAAW},
}

\bib{Kir}{article}{
	AUTHOR 	= {Kirchberg, Eberhard},
	TITLE	= {The classication of purely infinite C*-algebras using Kasparov's theory},
	JOURNAL = {to appear in Fields Inst. Commun, Amer. Math. Soc. Providence},
}

\bib{KK}{article}{
	AUTHOR = {Kalantar, Mehrdad},
	AUTHOR = {Kennedy, Matthew},
	TITLE  = {Boundaries of reduced C*-algebras of discrete groups},
	JOURNAL = {to appear in J. Reine Angew. Math.},
    NOTE 	= {preprint \href{http://arxiv.org/pdf/1405.4359v1}{arxiv:1405.4359v1}},
}

\bib{KP}{article}{
AUTHOR = {Kumjian, Alex},
author={Pask, David},
     TITLE = {Higher rank graph {$C^*$}-algebras},
   JOURNAL = {New York J. Math.},
%  FJOURNAL = {New York Journal of Mathematics},
    VOLUME = {6},
      YEAR = {2000},
     PAGES = {1--20},
      ISSN = {1076-9803},
   %MRCLASS = {46L35 (46L45)},
  %MRNUMBER = {1745529 (2001b:46102)},
%MRREVIEWER = {Michael Frank},
       URL = {\href{http://nyjm.albany.edu:8000/j/2000/6_1.html}{nyjm:8000/j/2000/6_1}},
}

%\bib{KPRR}{article} {%MR1432596,
 %   AUTHOR = {Kumjian, Alex},
 %   AUTHOR = {Pask, David},
 %   AUTHOR = {Raeburn, Iain},
 %   AUTHOR = {Renault, Jean},
 %    TITLE = {Graphs, groupoids, and {C}untz-{K}rieger algebras},
 %  JOURNAL = {J. Funct. Anal.},
 % FJOURNAL = {Journal of Functional Analysis},
 %   VOLUME = {144},
 %     YEAR = {1997},
 %   NUMBER = {2},
 %    PAGES = {505--541},
 %     ISSN = {0022-1236},
    % CODEN = {JFUAAW},
  % MRCLASS = {46L05 (46L55)},
 % MRNUMBER = {1432596 (98g:46083)},
%MRREVIEWER = {Masatoshi Enomoto},
  %     DOI = {10.1006/jfan.1996.3001},
  %     URL = {http://dx.doi.org/10.1006/jfan.1996.3001},
%}

\bib{Kri}{article} {%MR1934386,
    AUTHOR = {Kribs, David W.},
     TITLE = {Inductive limit algebras from periodic weighted shifts on {F}ock space},
   JOURNAL = {New York J. Math.},
%  FJOURNAL = {New York Journal of Mathematics},
    VOLUME = {8},
      YEAR = {2002},
     PAGES = {145--159 (electronic)},
      ISSN = {1076-9803},
%   MRCLASS = {46L05 (46L35)},
%  MRNUMBER = {1934386 (2004b:46073)},
%MRREVIEWER = {Il Bong Jung},
       NOTE = {\href{http://nyjm.albany.edu:8000/j/2002/8_145.html}{nyjm.albany.edu:8000/j/2002/8_145}},
}

\bib{KS}{article}{
author={Kwa\'{s}niewski, Bartosz},
author={Szyma\'{n}ski, Wojciech},
title={Topological aperiodicity for product systems over semigroups of Ore type},
note={preprint \href{http://arxiv.org/pdf/1312.7472v1}{arxiv:1312.7472v1}},
}

\bib{KT}{article}{%MR1088230,
    AUTHOR = {Kawamura, Shinz{\=o}},
    AUTHOR = {Tomiyama, Jun},
     TITLE = {Properties of topological dynamical systems and corresponding {$C^*$}-algebras},
   JOURNAL = {Tokyo J. Math.},
%  FJOURNAL = {Tokyo Journal of Mathematics},
    VOLUME = {13},
      YEAR = {1990},
    NUMBER = {2},
     PAGES = {251--257},
      ISSN = {0387-3870},
%   MRCLASS = {46L55 (54H20)},
%  MRNUMBER = {1088230 (92e:46131)},
%MRREVIEWER = {John Quigg},
       DOI = {\href{http://dx.doi.org/10.3836/tjm/1270132260}{10.3836/tjm/1270132260}},
 %      URL = ,
}

\bib{Laca98}{article}{%MR1608003,
    AUTHOR = {Laca, Marcelo},
     TITLE = {Semigroups of $*$-endomorphisms, {D}irichlet series, and phase transitions},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {152},
      YEAR = {1998},
    NUMBER = {2},
     PAGES = {330--378},
      ISSN = {0022-1236},
    % CODEN = {JFUAAW},
   %MRCLASS = {46L55 (11M41 46L40 82B26)},
  %MRNUMBER = {1608003},
       DOI = {\href{http://dx.doi.org/10.1006/jfan.1997.3166}{10.1006/jfan.1997.3166}},
      % URL = {http://dx.doi.org/10.1006/jfan.1997.3166},
}

\bib{Lac}{article}{
    AUTHOR = {Laca, Marcelo},
     TITLE = {From endomorphisms to automorphisms and back: dilations and full corners},
   JOURNAL = {J. London Math. Soc. (2)},
%  FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {61},
    YEAR = {2000},
    NUMBER = {3},
    PAGES = {893--904},
    DOI = {\href{http://dx.doi.org/10.1112/S0024610799008492}{10.1112/S0024610799008492}},
}

\bib{LaNe}{article} {%MR2785897,
    AUTHOR = {Laca, Marcelo},
    author={Neshveyev, Sergey},
     TITLE = {Type {$\rm III\sb 1$} equilibrium states of the {T}oeplitz algebra of the affine semigroup over the natural numbers},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {261},
      YEAR = {2011},
    NUMBER = {1},
     PAGES = {169--187},
      ISSN = {0022-1236},
     %CODEN = {JFUAAW},
   %MRCLASS = {46L55 (11M55 46L30)},
  %MRNUMBER = {2785897},
%MRREVIEWER = {Douglas R. Farenick},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2011.03.009}{10.1016/j.jfa.2011.03.009}},
  %     URL = {http://dx.doi.org/10.1016/j.jfa.2011.03.009},
}

\bib{LR1}{article}{
AUTHOR = {Laca, Marcelo},
author={Raeburn, Iain},
     TITLE = {Semigroup crossed products and the {T}oeplitz algebras of nonabelian groups},
   JOURNAL = {J. Funct. Anal.},
 % FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {139},
      YEAR = {1996},
    NUMBER = {2},
     PAGES = {415--440},
      ISSN = {0022-1236},
   %  CODEN = {JFUAAW},
  % MRCLASS = {46L55 (46L35 47B35)},
 % MRNUMBER = {1402771 (97h:46109)},
%MRREVIEWER = {Erik B{\'e}dos},
       DOI = {\href{http://dx.doi.org/10.1006/jfan.1996.0091}{10.1006/jfan.1996.0091}},
}

\bib{LR2}{article}{%MR2671177,
    AUTHOR = {Laca, Marcelo},
    author={Raeburn, Iain},
     TITLE = {Phase transition on the {T}oeplitz algebra of the affine semigroup over the natural numbers},
   JOURNAL = {Adv. Math.},
  %FJOURNAL = {Advances in Mathematics},
    VOLUME = {225},
      YEAR = {2010},
    NUMBER = {2},
     PAGES = {643--688},
      ISSN = {0001-8708},
     %CODEN = {ADMTA4},
   %MRCLASS = {46L55 (46L30)},
  %MRNUMBER = {2671177 (2012g:46102)},
%MRREVIEWER = {Erik B{\'e}dos},
       DOI = {\href{http://dx.doi.org/10.1016/j.aim.2010.03.007}{10.1016/j.aim.2010.03.007}},
%       URL = {http://dx.doi.org/10.1016/j.aim.2010.03.007},
}

\bib{LRR}{article}{%MR2838037,
    AUTHOR = {Laca, Marcelo},
    AUTHOR = {Raeburn, Iain},
    AUTHOR = {Ramagge, Jacqui},
     TITLE = {Phase transition on {E}xel crossed products associated to dilation matrices},
   JOURNAL = {J. Funct. Anal.},
  %FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {261},
      YEAR = {2011},
    NUMBER = {12},
     PAGES = {3633--3664},
      ISSN = {0022-1236},
     %CODEN = {JFUAAW},
   %MRCLASS = {46L30 (46L55)},
  %MRNUMBER = {2838037},
%MRREVIEWER = {Sriwulan Adji},
       DOI = {\href {http://dx.doi.org/10.1016/j.jfa.2011.08.015}{10.1016/j.jfa.2011.08.015}},
  %     URL = {http://dx.doi.org/10.1016/j.jfa.2011.08.015},
}

\bib{LRRW}{article}{%MR3192463,
    AUTHOR = {Laca, Marcelo},
    AUTHOR = {Raeburn, Iain},
    AUTHOR = {Ramagge, Jacqui},
    AUTHOR = {Whittaker, Michael F.},
     TITLE = {Equilibrium states on the {C}untz-{P}imsner algebras of self-similar actions},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {266},
      YEAR = {2014},
    NUMBER = {11},
     PAGES = {6619--6661},
      ISSN = {0022-1236},
%   MRCLASS = {46L30 (46L55)},
 % MRNUMBER = {3192463},
%MRREVIEWER = {Mark Tomforde},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2014.03.003}{10.1016/j.jfa.2014.03.003}},
     %  URL = {http://dx.doi.org/10.1016/j.jfa.2014.03.003},
}

\bib{LRRW1}{article}{%MR3192463,
    AUTHOR = {Laca, Marcelo},
    AUTHOR = {Raeburn, Iain},
    AUTHOR = {Ramagge, Jacqui},
    AUTHOR = {Whittaker, Michael F.},
     TITLE = {Equilibrium states on operator algebras associated to self-similar actions of groupoids on graphs},
     NOTE={preprint, \href{http://arxiv.org/abs/1610.00343}{arxiv.org:1610.00343}}
   %JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
   % VOLUME = {266},
    %  YEAR = {2014},
    %NUMBER = {11},
     %PAGES = {6619--6661},
     % ISSN = {0022-1236},
%   MRCLASS = {46L30 (46L55)},
 % MRNUMBER = {3192463},
%MRREVIEWER = {Mark Tomforde},
      % DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2014.03.003}{10.1016/j.jfa.2014.03.003}},
     %  URL = {http://dx.doi.org/10.1016/j.jfa.2014.03.003},
}

\bib{Lan}{book}{%MR1325694,
    AUTHOR = {Lance, Christopher E.},
     TITLE = {Hilbert C*-Modules},
    SERIES = {London Mathematical Society Lecture Note Series},
    VOLUME = {210},
   %   NOTE = {A Toolkit for Operator Algebraists},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {1995},
     PAGES = {x+130},
      ISBN = {0-521-47910-X},
  % MRCLASS = {46L05 (46H25 46K05 46L80 46M05 47D25)},
 % MRNUMBER = {1325694 (96k:46100)},
%MRREVIEWER = {Robert S. Doran},
       DOI = {\href{http://dx.doi.org/10.1017/CBO9780511526206}{10.1017/CBO9780511526206}},
}

\bib{Lar}{article} {%MR2669415,
    AUTHOR = {Larsen, Nadia S.},
     TITLE = {Crossed products by abelian semigroups via transfer operators},
   JOURNAL = {Ergodic Theory Dynam. Systems},
%  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {30},
      YEAR = {2010},
    NUMBER = {4},
     PAGES = {1147--1164},
      ISSN = {0143-3857},
%   MRCLASS = {46L55},
%  MRNUMBER = {2669415 (2011j:46114)},
%MRREVIEWER = {Sriwulan Adji},
       DOI = {\href{http://dx.doi.org/10.1017/S0143385709000509}{10.1017/S0143385709000509}},
}

\bib{LarsenLi}{article}{
    AUTHOR = {Larsen, Nadia S.},
    author = {Li, Xin},
     TITLE = {The $2$-adic ring {$C^*$}-algebra of the integers and its representations},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {262},
      YEAR = {2012},
    NUMBER = {4},
     PAGES = {1392--1426},
}

\bib{LR}{article} {%MR2339372,
    AUTHOR = {Larsen, Nadia S.},
    AUTHOR = {Raeburn, Iain},
     TITLE = {Projective multi-resolution analyses arising from direct limits of {H}ilbert modules},
   JOURNAL = {Math. Scand.},
%  FJOURNAL = {Mathematica Scandinavica},
    VOLUME = {100},
      YEAR = {2007},
    NUMBER = {2},
     PAGES = {317--360},
      ISSN = {0025-5521},
%     CODEN = {MTSCAN},
%   MRCLASS = {42C40 (28A80 46C05 46H25 46L08 60D05)},
%  MRNUMBER = {2339372 (2008m:42059)},
%MRREVIEWER = {Palle E. T. Jorgensen},
}

\bib{Law1}{article}{%MR2395198,
    AUTHOR = {Lawson, Mark V.},
     TITLE = {A correspondence between a class of monoids and self-similar group actions. {I}},
   JOURNAL = {Semigroup Forum},
  %FJOURNAL = {Semigroup Forum},
    VOLUME = {76},
      YEAR = {2008},
    NUMBER = {3},
     PAGES = {489--517},
      ISSN = {0037-1912},
     %CODEN = {SMGFAN},
   %MRCLASS = {20M20 (20M18)},
  %MRNUMBER = {2395198},
%MRREVIEWER = {P. M. Higgins},
       DOI = {\href{http://dx.doi.org/10.1007/s00233-008-9052-x}{10.1007/s00233-008-9052-x}},
  %     URL = {http://dx.doi.org/10.1007/s00233-008-9052-x},
}


\bib{Law2}{article}{%MR2395198,
    AUTHOR = {Lawson, Mark V.},
     TITLE = {Non-commutative Stone duality: inverse semigroups, topological groupoids and $C^*$-algebras},
   JOURNAL = {Internat. J. Algebra Comput.},
    VOLUME = {22},
      YEAR = {2012},
    NUMBER = {6},
     PAGES = {1250058, 47 pp.}
     }

\bib{Li0}{article}{%MR2721644,
    AUTHOR = {Li, Xin},
     TITLE = {Ring C*-algebras},
   JOURNAL = {Math. Ann.},
 % FJOURNAL = {Mathematische Annalen},
    VOLUME = {348},
      YEAR = {2010},
    NUMBER = {4},
     PAGES = {859--898},
      ISSN = {0025-5831},
   %  CODEN = {MAANA},
  % MRCLASS = {46L05 (11R56 16D30 58B34)},
 % MRNUMBER = {2721644 (2012a:46100)},
%MRREVIEWER = {Nadia S. Larsen},
       DOI = {\href{http://dx.doi.org/10.1007/s00208-010-0502-x}{10.1007/s00208-010-0502-x}},
}

\bib{Li1}{article} {%MR2900468,
    AUTHOR = {Li, Xin},
     TITLE = {Semigroup {$C^*$}-algebras and amenability of semigroups},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {262},
      YEAR = {2012},
    NUMBER = {10},
     PAGES = {4302--4340},
      ISSN = {0022-1236},
%     CODEN = {JFUAAW},
%   MRCLASS = {46L05},
%  MRNUMBER = {2900468},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2012.02.020}{10.1016/j.jfa.2012.02.020}},
}

\bib{Li2}{article}{%MR3077884,
    AUTHOR = {Li, Xin},
     TITLE = {Nuclearity of semigroup C*-algebras and the connection to amenability},
   JOURNAL = {Adv. Math.},
%  FJOURNAL = {Advances in Mathematics},
    VOLUME = {244},
      YEAR = {2013},
     PAGES = {626--662},
      ISSN = {0001-8708},
%   MRCLASS = {46L05 (20M12 43A07)},
%  MRNUMBER = {3077884},
%MRREVIEWER = {Takahiro Sudo},
       DOI = {\href{http://dx.doi.org/10.1016/j.aim.2013.05.016}{10.1016/j.aim.2013.05.016}},
}

\bib{LN2}{article}{
    author = {Li, Xin},
    author={Norling, Magnus},
    title  = {Independent resolutions for totally disconnected dynamical systems. {II}. {$C^*$}-algebraic case},
    journal={J. Op. Th.},
    volume={75},
    number={1},
    year={2016},
    pages={163--193},
   doi={\href{http://www.mathjournals.org/jot/2016-075-001/2016-075-001-009.html}{10.7900/jot.2014dec22.2061}},
}

\bib{Lin}{article}{%MR1814969,
    AUTHOR = {Lin, Huaxin},
     TITLE = {Classification of simple tracially {AF} C*-algebras},
   JOURNAL = {Canad. J. Math.},
%  FJOURNAL = {Canadian Journal of Mathematics. Journal Canadien de Math\'{e}matiques},
    VOLUME = {53},
      YEAR = {2001},
    NUMBER = {1},
     PAGES = {161--194},
      ISSN = {0008-414X},
   %  CODEN = {CJMAAB},
  % MRCLASS = {46L35 (19K14 46L05 46L80)},
 % MRNUMBER = {1814969 (2002h:46102)},
%MRREVIEWER = {Judith A. Packer},
       DOI = {\href{http://dx.doi.org/10.4153/CJM-2001-007-8}{10.4153/CJM-2001-007-8}},
}

\bib{LS}{incollection} {%MR1928527,
    AUTHOR = {Lind, Douglas},
    AUTHOR = {Schmidt, Klaus},
     TITLE = {Symbolic and algebraic dynamical systems},
 BOOKTITLE = {Handbook of dynamical systems, {V}ol.\ 1{A}},
     PAGES = {765--812},
 PUBLISHER = {North-Holland, Amsterdam},
      YEAR = {2002},
   %MRCLASS = {37B50 (37A15 37B10)},
  %MRNUMBER = {1928527 (2003h:37017)},
%MRREVIEWER = {Anthony Quas},
       DOI = {\href{http://dx.doi.org/10.1016/S1874-575X(02)80012-1}{10.1016/S1874-575X(02)80012-1}},
 %      URL = ,
}


\bib{massey1}{article}{
author={Massey, W. S.},
title={{Exact couples in algebraic topology (Parts I \& II)}},
year={1952},
journal={Ann. Math.},
volume={56},
pages={363--396}
}

\bib{massey2}{article}{
author={Massey, W. S.},
title={{Exact couples in algebraic topology (Parts III, IV \& V)}},
year={1953},
journal={Ann. Math.},
volume={57},
pages={248--286}
}

\bib{Mat}{article} {%MR1774695,
    AUTHOR = {Matsumoto, Kengo},
     TITLE = {On automorphisms of C*-algebras associated with subshifts},
   JOURNAL = {J. Operator Theory},
  %FJOURNAL = {Journal of Operator Theory},
    VOLUME = {44},
      YEAR = {2000},
    NUMBER = {1},
     PAGES = {91--112},
      ISSN = {0379-4024}
  % MRCLASS = {46L55 (37A55 37B10)},
 % MRNUMBER = {1774695 (2001g:46147)},
%MRREVIEWER = {A. I. Danilenko},
}

\bib{MS}{article}{
	AUTHOR 	= {Matui, Hiroki},
	AUTHOR 	= {Sato, Yasuhiko},
	TITLE 	= {Decomposition rank of UHF-absorbing C*-algebras},
	JOURNAL	= {Duke Math. J.},
	DOI = {\href{http://dx.doi.org/10.1215/00127094-2826908}{10.1215/00127094-2826908}},
%journal = {Duke Mathematical Journal},
%month = {11},
	pages = {2687--2708},
	volume = {163},
	number = {14},
	year = {2014},
}

\bib{MW}{article}{
	AUTHOR 	= {Maloney, Ben},
	AUTHOR 	= {Willis, Paulette N.},
	TITLE 	= {Examples of $*$-commuting maps},
	%JOURNAL	= {preprint},
    NOTE 	= {preprint \href{http://arxiv.org/abs/1101.3795v2}{arxiv:1101.3795v2}},	
}

\bib{Muc}{article}{%MR2136018,
    AUTHOR = {Muchnik, Roman},
     TITLE = {Semigroup actions on $\IT^n$},
   JOURNAL = {Geom. Dedicata},
  %FJOURNAL = {Geometriae Dedicata},
    VOLUME = {110},
      YEAR = {2005},
     PAGES = {1--47},
      ISSN = {0046-5755},
   %  CODEN = {GEMDAT},
  % MRCLASS = {37B05 (20M20)},
 % MRNUMBER = {2136018 (2006i:37022)},
%MRREVIEWER = {Daniel Berend},
}

\bib{Nek1}{book}{%MR2162164,
    AUTHOR = {Nekrashevych, Volodymyr},
     TITLE = {Self-similar groups},
    SERIES = {Mathematical Surveys and Monographs},
    VOLUME = {117},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {2005},
     PAGES = {xii+231},
      ISBN = {0-8218-3831-8},
  % MRCLASS = {20E08 (20F65 37B15 37F10)},
  %MRNUMBER = {2162164},
%MRREVIEWER = {Laurent Bartholdi},
       DOI = {\href{http://dx.doi.org/10.1090/surv/117}{10.1090/surv/117}},
    %   URL = {http://dx.doi.org/10.1090/surv/117},
}

\bib{Nes}{article}{%MR3138368,
    AUTHOR = {Neshveyev, Sergey},
     TITLE = {K{MS} states on the {$C\sp \ast$}-algebras of non-principal groupoids},
   JOURNAL = {J. Operator Theory},
  %FJOURNAL = {Journal of Operator Theory},
    VOLUME = {70},
      YEAR = {2013},
    NUMBER = {2},
     PAGES = {513--530},
      ISSN = {0379-4024},
  % MRCLASS = {46L30 (46L55)},
 % MRNUMBER = {3138368},
%MRREVIEWER = {Massoud Amini},
       DOI = {\href{http://dx.doi.org/10.7900/jot.2011sep20.1915}{10.7900/jot.2011sep20.1915}},
  %     URL = {http://dx.doi.org/10.7900/jot.2011sep20.1915},
}

\bib{Neu}{article}{%MR0062122,
    AUTHOR = {Neumann, B. H.},
     TITLE = {Groups covered by permutable subsets},
   JOURNAL = {J. London Math. Soc.},
  %FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {29},
      YEAR = {1954},
     PAGES = {236--248},
      ISSN = {0024-6107},
   %MRCLASS = {20.0X},
  %MRNUMBER = {0062122 (15,931b)},
%MRREVIEWER = {D. G. Higman},
}

\bib{Nic}{article}{%MR1241114,
    AUTHOR = {Nica, Alexandru},
     TITLE = {C*-algebras generated by isometries and {W}iener-{H}opf operators},
   JOURNAL = {J. Operator Theory},
 % FJOURNAL = {Journal of Operator Theory},
    VOLUME = {27},
      YEAR = {1992},
    NUMBER = {1},
     PAGES = {17--52},
      ISSN = {0379-4024},
  % MRCLASS = {46L35 (47B35 47C10)},
 % MRNUMBER = {1241114 (94m:46094)},
%MRREVIEWER = {Ra{\'u}l E. Curto},
}


\bib{NS}{book} {%MR2251116,				%%%notwendig? Walters als Referenz!
    AUTHOR = {Neshveyev, Sergey},
    AUTHOR = {St{\o}rmer, Erling},
     TITLE = {Dynamical Entropy in Operator Algebras},
    SERIES = {Ergebnisse der Mathematik und ihrer Grenzgebiete. 3. Folge. A Series of Modern Surveys in Mathematics [Results in Mathematics and Related Areas. 3rd Series. A Series of Modern Surveys in Mathematics]},
    VOLUME = {50},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin},
      YEAR = {2006},
     PAGES = {x+296},
      ISBN = {978-3-540-34670-8; 3-540-34670-8}
   %MRCLASS = {46L55 (28D20 37B40 46L54 82C10)},
  %MRNUMBER = {2251116 (2007m:46108)},
%MRREVIEWER = {Adam G. Skalski}
}

\bib{Nor1}{article}{%MR3200323,
    AUTHOR = {Norling, Magnus Dahler},
     TITLE = {Inverse semigroup {$C\sp *$}-algebras associated with left cancellative semigroups},
   JOURNAL = {Proc. Edinb. Math. Soc. (2)},
  %FJOURNAL = {Proceedings of the Edinburgh Mathematical Society. Series II},
    VOLUME = {57},
      YEAR = {2014},
    NUMBER = {2},
     PAGES = {533--564},
      ISSN = {0013-0915},
%   MRCLASS = {46L05 (06F15 20M18 43A07)},
%  MRNUMBER = {3200323},
%MRREVIEWER = {Camillo Trapani},
       DOI = {\href{http://dx.doi.org/10.1017/S0013091513000540}{10.1017/S0013091513000540}},
%       URL = {http://dx.doi.org/10.1017/S0013091513000540},
}


\bib{olesenPedersen}{article}{
author={Olesen, D.},
author={Pedersen, G. K.},
title={{Partially Inner {$C^{*}$}-dynamical Systems}},
year={1986},
journal={J. Funct. Anal.},
volume={66},
number={2},
pages={262--281}
}

\bib{Oml}{incollection}{%MR3142039,
    AUTHOR = {Omland, Tron},
     TITLE = {{$C\sp *$}-algebras associated with {$a$}-adic numbers},
 BOOKTITLE = {Operator algebra and dynamics},
    SERIES = {Springer Proc. Math. Stat.},
    VOLUME = {58},
     PAGES = {223--238},
 PUBLISHER = {Springer, Heidelberg},
      YEAR = {2013},
   %MRCLASS = {46L55 (11S82)},
  %MRNUMBER = {3142039},
%MRREVIEWER = {Marius V. Ionescu},
       DOI = {\href{http://dx.doi.org/10.1007/978-3-642-39459-1_11}{$10.1007/978-3-642-39459-1_11$}},
     %  URL = ,
}

\bib{Orf}{article} {%MR2550195,
    AUTHOR = {Orfanos, Stefanos},
     TITLE = {Generalized {B}unce-{D}eddens algebras},
   JOURNAL = {Proc. Amer. Math. Soc.},
%  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {138},
      YEAR = {2010},
    NUMBER = {1},
     PAGES = {299--308},
      ISSN = {0002-9939},
%     CODEN = {PAMYAR},
%   MRCLASS = {46L55 (46L05 47L65)},
%  MRNUMBER = {2550195 (2011a:46104)},
%MRREVIEWER = {Michal Zajac},
       DOI = {\href{http://dx.doi.org/10.1090/S0002-9939-09-10071-0}{10.1090/S0002-9939-09-10071-0}},
}

\bib{Oza}{article}{%MR1763912,
    AUTHOR = {Ozawa, Narutaka},
     TITLE = {Amenable actions and exactness for discrete groups},
   JOURNAL = {C. R. Acad. Sci. Paris S\'{e}r. I Math.},
%  FJOURNAL = {Comptes Rendus de l'Acad\'emie des Sciences. S\'erie I.Math\'ematique},
    VOLUME = {330},
      YEAR = {2000},
    NUMBER = {8},
     PAGES = {691--695},
      ISSN = {0764-4442},
   %  CODEN = {CASMEI},
  % MRCLASS = {22D25 (43A35 46L06 46L55)},
 % MRNUMBER = {1763912 (2001g:22007)},
%MRREVIEWER = {Alain Valette},
       DOI = {\href{http://dx.doi.org/10.1016/S0764-4442(00)00248-2}{10.1016/S0764-4442(00)00248-2}},
}

\bib{Par}{incollection}{%MR1411219,
    AUTHOR = {Parry, William},
     TITLE = {Squaring and cubing the circle \mdash {R}udolph's theorem},
 BOOKTITLE = {Ergodic theory of $\Z^d$-actions ({W}arwick,
              1993--1994)},
    SERIES = {London Math. Soc. Lecture Note Ser.},
    VOLUME = {228},
     PAGES = {177--183},
 PUBLISHER = {Cambridge Univ. Press, Cambridge},
      YEAR = {1996},
  % MRCLASS = {28D15 (11K16)},
 % MRNUMBER = {1411219 (97h:28009)},
%MRREVIEWER = {Thomas Ward},
       DOI = {\href{http://dx.doi.org/10.1017/CBO9780511662812.006}{10.1017/CBO9780511662812.006}},
}

\bib{Phi}{article} {%MR1745197,
    AUTHOR = {Phillips, Christopher N.},
     TITLE = {A classification theorem for nuclear purely infinite simple C*-algebras},
   JOURNAL = {Doc. Math.},
  %FJOURNAL = {Documenta Mathematica},
    VOLUME = {5},
      YEAR = {2000},
     PAGES = {49--114 (electronic)},
      ISSN = {1431-0635},
 %  MRCLASS = {46L05 (19K56 46L35 46L80)},
  %MRNUMBER = {1745197 (2001d:46086b)},
%MRREVIEWER = {Mikael R{\o}rdam},
}

\bib{Pim}{incollection} {%MR1426840,
    AUTHOR = {Pimsner, Mihai V.},
     TITLE = {A class of C*-algebras generalizing both {C}untz-{K}rieger algebras and crossed products by $\Z$},
 BOOKTITLE = {Free probability theory ({W}aterloo, {ON}, 1995)},
    SERIES = {Fields Inst. Commun.},
    VOLUME = {12},
     PAGES = {189--212},
 PUBLISHER = {Amer. Math. Soc.},
   ADDRESS = {Providence, RI},
      YEAR = {1997},
  % MRCLASS = {46L05 (46L55 46L80)},
 % MRNUMBER = {1426840 (97k:46069)},
%MRREVIEWER = {Michael Frank},
}

\bib{PV}{article}{
	Author = {Pimsner, Mihai V.},
	Author = {Voiculescu, Dan-Virgil},
	TITLE = {Exact sequences for $K$-groups and Ext-groups of certain cross-product $C^*$-algebras},
	JOURNAL = {J. Operator Theory},
	VOLUME = {4},
	NUMBER = {1},
	YEAR = {1980},
	PAGES = {93--118},
}

\bib{PR}{article} {%MR1964302,
    AUTHOR = {Packer, Judith A.},
    AUTHOR = {Rieffel, Marc A.},
     TITLE = {Wavelet filter functions, the matrix completion problem, and modules over $C(\IT^n)$},
   JOURNAL = {J. Fourier Anal. Appl.},
  %FJOURNAL = {The Journal of Fourier Analysis and Applications},
    VOLUME = {9},
      YEAR = {2003},
    NUMBER = {2},
     PAGES = {101--116},
      ISSN = {1069-5869},
  % MRCLASS = {42C40 (46H25 46L99 94A12)},
 % MRNUMBER = {1964302 (2003m:42063)},
%MRREVIEWER = {Jo Ward},
       DOI = {\href{http://dx.doi.org/10.1007/s00041-003-0010-4}{10.1007/s00041-003-0010-4}},
}

\bib{RW}{book}{%MR1634408,
    AUTHOR = {Raeburn, Iain},
    author={Williams, Dana P.},
     TITLE = {Morita equivalence and continuous-trace {$C\sp *$}-algebras},
    SERIES = {Mathematical Surveys and Monographs},
    VOLUME = {60},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {1998},
     PAGES = {xiv+327},
      ISBN = {0-8218-0860-5},
%   MRCLASS = {46L05 (22D99 46L55 46M20)},
%  MRNUMBER = {1634408},
%MRREVIEWER = {Robert S. Doran},
       DOI = {\href{10.1090/surv/060}{http://dx.doi.org/10.1090/surv/060}},
    %   URL = {http://dx.doi.org/10.1090/surv/060},
}



\bib{RS}{article}{
	AUTHOR = {Raeburn, Iain},
	AUTHOR = {Szyma{\'n}ski, Wojciech}
	TITLE = {Cuntz-Krieger algebras of infinite graphs and matrices},
	JOURNAL = {Trans. Amer. Math. Soc.},
	VOLUME = {356},
	NUMBER = {1},
	PAGES = {39--59},
	YEAR = {2004},
}

%Referenz im Ausblick zu den Bereichen, die helfen könnten.
%\bib{R}{book} {%MR584266,
 %   AUTHOR = {Renault, Jean},
 %    TITLE = {A groupoid approach to {$C\sp{\ast} $}-algebras},
 %   SERIES = {Lecture Notes in Mathematics},
 %   VOLUME = {793},
% PUBLISHER = {Springer},
%   ADDRESS = {Berlin},
%      YEAR = {1980},
%     PAGES = {ii+160},
%      ISBN = {3-540-09977-8},
  % MRCLASS = {46Lxx (22D25 22D40)},
  %MRNUMBER = {584266 (82h:46075)},
%MRREVIEWER = {A. K. Seda},
%}

\bib{rordam}{article}{
    AUTHOR = {R{\o}rdam, Mikael},
     TITLE = {Classification of certain infinite simple {$C^*$}-algebras},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {131},
      YEAR = {1995},
    NUMBER = {2},
     PAGES = {415--458},
      ISSN = {0022-1236},
     %CODEN = {JFUAAW},
   %MRCLASS = {46L05 (19K35 46L35 46L80)},
 % MRNUMBER = {1345038 (96e:46080a)},
%MRREVIEWER = {Judith A. Packer},
       DOI = {\href{http://dx.doi.org/10.1006/jfan.1995.1095}{10.1006/jfan.1995.1095}},
%       URL = ,
}

\bib{Rud}{article} {%MR1062766,
    AUTHOR = {Rudolph, Daniel J.},
     TITLE = {{$\times 2$} and {$\times 3$} invariant measures and entropy},
   JOURNAL = {Ergodic Theory Dynam. Systems},
  %FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {10},
      YEAR = {1990},
    NUMBER = {2},
     PAGES = {395--406},
      ISSN = {0143-3857},
  % MRCLASS = {28D20},
  %MRNUMBER = {1062766 (91g:28026)},
%MRREVIEWER = {Ladislav Andrey},
      DOI = {\href{http://dx.doi.org/10.1017/S0143385700005629}{10.1017/S0143385700005629}},
}

%\bib{RL}{book} {%MR1783408,
 %   AUTHOR = {R{\o}rdam, M.},
  %  AUTHOR = {Larsen, F.},
   % AUTHOR = {Laustsen, N.},
    % TITLE = {An introduction to {$K$}-theory for C*-algebras},
    %SERIES = {London Mathematical Society Student Texts},
    %VOLUME = {49},
 %PUBLISHER = {Cambridge University Press},
 %  ADDRESS = {Cambridge},
  %    YEAR = {2000},
   %  PAGES = {xii+242},
    %  ISBN = {0-521-78334-8; 0-521-78944-3}
  % MRCLASS = {46-01 (19K35 46L80)},
 % MRNUMBER = {1783408 (2001g:46001)},
%MRREVIEWER = {{\'E}ric Leichtnam},
%}


%\bib{RS}{article} {%MR1713322,
 %   AUTHOR = {Robertson, Guyan},
  %  AUTHOR = {Steger, Tim},
   %  TITLE = {Affine buildings, tiling systems and higher rank
    %          {C}untz-{K}rieger algebras},
   %JOURNAL = {J. Reine Angew. Math.},
  %FJOURNAL = {Journal f\"ur die Reine und Angewandte Mathematik},
    %VOLUME = {513},
     % YEAR = {1999},
     %PAGES = {115--144},
     % ISSN = {0075-4102},
   %  CODEN = {JRMAA8},
  % MRCLASS = {46L05 (20E42 46L55)},
 % MRNUMBER = {1713322 (2000j:46109)},
%MRREVIEWER = {Claudia Pinzari},
      % DOI = {10.1515/crll.1999.057},
       %URL = {http://dx.doi.org/10.1515/crll.1999.057}
%}

\bib{savinienBellissard}{article}{
author={Savinien, J.},
author = {Bellissard, J.},
title={{A spectral sequence for the {$K$}-theory of tiling spaces}},
year={2009},
journal={{Ergod. Th. \& Dynam. Sys.}},
volume={29},
pages={997--1031}
}

\bib{Sch1}{book} {%MR3024809,
    AUTHOR = {Schmidt, Klaus},
     TITLE = {Dynamical systems of algebraic origin},
    SERIES = {Modern Birkh\"auser Classics},
%      NOTE = {[2011 reprint of the 1995 original]},% [MR1345152]},
 PUBLISHER = {Birkh\"auser/Springer Basel AG, Basel},
      YEAR = {1995},
     PAGES = {xviii+310},
      ISBN = {978-3-0348-0276-5; 978-3-0348-0277-2},
   %MRCLASS = {01A75},
 % MRNUMBER = {3024809},
}

\bib{Sch2}{incollection} {%MR1905342,
    AUTHOR = {Schmidt, Klaus},
     TITLE = {The dynamics of algebraic {$\Z^d$}-actions},
 BOOKTITLE = {European {C}ongress of {M}athematics, {V}ol. {I} ({B}arcelona,
              2000)},
    SERIES = {Progr. Math.},
    VOLUME = {201},
     PAGES = {543--553},
 PUBLISHER = {Birkh\"auser, Basel},
      YEAR = {2001},
   %MRCLASS = {37A15 (28D20)},
  %MRNUMBER = {1905342 (2003e:37007)},
%MRREVIEWER = {Thomas Ward},
}

\bib{schochet}{article}{
author={Schochet, C.},
title={{Topological methods for {$C^*$}-algebras I: Spectral sequences}},
year={1981},
journal={Pacific J. Math.},
volume={96},
number={1},
pages={193--211},
}

\bib{Sie}{article}{%MR2775364,
    AUTHOR = {Sierakowski, Adam},
     TITLE = {The ideal structure of reduced crossed products},
   JOURNAL = {M\"unster J. Math.},
  %FJOURNAL = {M\"unster Journal of Mathematics},
    VOLUME = {3},
      YEAR = {2010},
     PAGES = {237--261},
      ISSN = {1867-5778},
  % MRCLASS = {46L55 (22D25)},
 % MRNUMBER = {2775364 (2012g:46103)},
%MRREVIEWER = {Tomoyoshi Ohwada},
}


%\bib{Sim}{article} {%MR2270926,
 %   AUTHOR = {Sims, Aidan},
  %   TITLE = {Gauge-invariant ideals in the {$C\sp *$}-algebras of finitely
   %           aligned higher-rank graphs},
   %JOURNAL = {Canad. J. Math.},
  %FJOURNAL = {Canadian Journal of Mathematics. Journal Canadien de
%              Math\'ematiques},
%    VOLUME = {58},
 %     YEAR = {2006},
  %  NUMBER = {6},
   %  PAGES = {1268--1290},
    %  ISSN = {0008-414X},
   %  CODEN = {CJMAAB},
   %MRCLASS = {46L05},
  %MRNUMBER = {2270926 (2007j:46095)},
%MRREVIEWER = {Bernhard Burgstaller},
     %  URL = {http://journals.cms.math.ca/ams/ams-redirect.php?Journal=CJM&Volume=58&FirstPage=1268}
%}

\bib{Sch3}{incollection} {%MR2090771,
    AUTHOR = {Schmidt, Klaus},
     TITLE = {Algebraic $\Z^d$-actions on zero-dimensional compact abelian groups},
 BOOKTITLE = {Modern dynamical systems and applications},
     PAGES = {185--209},
 PUBLISHER = {Cambridge Univ. Press, Cambridge},
      YEAR = {2004},
  % MRCLASS = {37A15 (28D15 34A45 37A25 37A35)},
 % MRNUMBER = {2090771 (2005g:37003)},
%MRREVIEWER = {Manfred Einsiedler},
}

\bib{Sol}{article}{%MR2225464,
    AUTHOR = {Solel, Baruch},
     TITLE = {Representations of product systems over semigroups and dilations of commuting {CP} maps},
   JOURNAL = {J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {235},
      YEAR = {2006},
    NUMBER = {2},
     PAGES = {593--618},
      ISSN = {0022-1236},
%     CODEN = {JFUAAW},
%   MRCLASS = {46L08 (46L57 47A20)},
%  MRNUMBER = {2225464 (2007h:46073)},
%MRREVIEWER = {B. V. Rajarama Bhat},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2005.11.014}{10.1016/j.jfa.2005.11.014}},
}

\bib{Spi1}{article}{%MR3000828,
    AUTHOR = {Spielberg, Jack},
     TITLE = {{$C\sp \ast$}-algebras for categories of paths associated to the {B}aumslag-{S}olitar groups},
   JOURNAL = {J. Lond. Math. Soc. (2)},
  %FJOURNAL = {Journal of the London Mathematical Society. Second Series},
    VOLUME = {86},
      YEAR = {2012},
    NUMBER = {3},
     PAGES = {728--754},
      ISSN = {0024-6107},
   %MRCLASS = {46L05 (46L55 46L80)},
  %MRNUMBER = {3000828},
%MRREVIEWER = {Mark Tomforde},
       DOI = {\href{http://dx.doi.org/10.1112/jlms/jds025}{10.1112/jlms/jds025}},
       %URL = {http://dx.doi.org/10.1112/jlms/jds025},
}

\bib{Stac}{article}{%MR1200792,
    AUTHOR = {Stacey, Peter J.},
     TITLE = {Crossed products of C*-algebras by {$\ast$}-endomorphisms},
   JOURNAL = {J. Austral. Math. Soc. Ser. A},
  %FJOURNAL = {Australian Mathematical Society. Journal. Series A. Pure Mathematics and Statistics},
    VOLUME = {54},
      YEAR = {1993},
    NUMBER = {2},
     PAGES = {204--212},
      ISSN = {0263-6115},
   %  CODEN = {JAMADS},
  % MRCLASS = {46L05 (46L55)},
 % MRNUMBER = {1200792 (94a:46077)},
%MRREVIEWER = {Shuang Zhang},
}

\bib{Sta1}{article}{
AUTHOR={Stammeier, Nicolai},
TITLE={On $C^*$-algebras of irreversible algebraic dynamical systems},
journal={J. Funct. Anal.},
%FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {269},
      YEAR = {2015},
    NUMBER = {4},
     PAGES = {1136--1179},
      %ISSN = {0022-1236},
   %MRCLASS = {46L55 (37A55)},
  %MRNUMBER = {3352767},
%MRREVIEWER = {Xin Li},
doi={\href{http://dx.doi.org/10.1016/j.jfa.2015.02.005}{10.1016/j.jfa.2015.02.005}},
 %     URL = {http://dx.doi.org/10.1016/j.jfa.2015.02.005},
}

\bib{Sta2}{article}{
	AUTHOR={Stammeier, Nicolai},
	TITLE={Topological freeness for $*$-commuting covering maps},
	NOTE={preprint, \href{http://arxiv.org/abs/1311.0793}{arxiv:1311.0793}},
}

\bib{Sta3}{article}{
	AUTHOR={Stammeier, Nicolai},
	TITLE={A boundary quotient diagram for right LCM semigroups},
	NOTE={preprint, \href{http://arxiv.org/abs/1604.03172}{arxiv:1604.03172}},
}

\bib{Star}{article}{
author={Starling, Charles},
label={Star15},
title={Boundary quotients of $C^*$-algebras of right LCM semigroups},
journal={J. Funct. Anal.},
%  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {268},
      YEAR = {2015},
    NUMBER = {11},
     PAGES = {3326--3356},
   %   ISSN = {0022-1236},
%   MRCLASS = {46L35},
 % MRNUMBER = {3336727},
%MRREVIEWER = {Camillo Trapani},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2015.01.001}{10.1016/j.jfa.2015.01.001}},
%       URL = {http://dx.doi.org/10.1016/j.jfa.2015.01.001},
}

\bib{ST}{article}{%MR2498769,
    AUTHOR = {Svensson, Christian},
    AUTHOR = {Tomiyama, Jun},
     TITLE = {On the commutant of {$C(X)$} in {$C^*$}-crossed products by {$\Z$} and their representations},
   JOURNAL = {J. Funct. Anal.},
  %FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {256},
      YEAR = {2009},
    NUMBER = {7},
     PAGES = {2367--2386},
      ISSN = {0022-1236},
   %  CODEN = {JFUAAW},
  % MRCLASS = {46L55},
 % MRNUMBER = {2498769 (2010f:46105)},
%MRREVIEWER = {Steven P. Kaliszewski},
       DOI = {\href{http://dx.doi.org/10.1016/j.jfa.2009.02.002}{10.1016/j.jfa.2009.02.002}},
       %URL = ,
}

\bib{SY}{article} {%MR2718947,
    AUTHOR = {Sims, Aidan},
    AUTHOR = {Yeend, Trent},
     TITLE = {C*-algebras associated to product systems of {H}ilbert bimodules},
   JOURNAL = {J. Operator Theory},
%  FJOURNAL = {Journal of Operator Theory},
    VOLUME = {64},
      YEAR = {2010},
    NUMBER = {2},
     PAGES = {349--376},
      ISSN = {0379-4024},
%   MRCLASS = {46L05 (46L08)},
%  MRNUMBER = {2718947 (2011j:46092)},
%MRREVIEWER = {Vladimir Manuilov},
}

%\bib{SZ}{article} {%MR2383707,
 %   AUTHOR = {Skalski, Adam},
  %  AUTHOR = {Zacharias, Joachim},
  %   TITLE = {Entropy of shifts on higher-rank graph {$C\sp *$}-algebras},
  % JOURNAL = {Houston J. Math.},
  %FJOURNAL = {Houston Journal of Mathematics},
   % VOLUME = {34},
    %  YEAR = {2008},
    %NUMBER = {1},
    % PAGES = {269--282},
    %  ISSN = {0362-1588},
    % CODEN = {HJMADZ},
   %MRCLASS = {46L55 (37B10 37B40)},
 % MRNUMBER = {2383707 (2009j:46165)},
%MRREVIEWER = {Aidan D. Sims}
%}

\bib{takai}{article}{
  title={{On a duality for crossed products by  {$C^*$}-algebras}},
  author={Takai, H.},
  journal={J. Funct. Anal.},
volume={19},
  year={1975},
  pages={25--39},
}

\bib{Tu}{article} {%MR1703305,
    AUTHOR = {Tu, Jean-Louis},
     TITLE = {La conjecture de {B}aum-{C}onnes pour les feuilletages moyennables},
   JOURNAL = {$K$-Theory},
 % FJOURNAL = {$K$-Theory. An Interdisciplinary Journal for the Development,
  %            Application, and Influence of $K$-Theory in the Mathematical
   %           Sciences},
    VOLUME = {17},
      YEAR = {1999},
    NUMBER = {3},
     PAGES = {215--264},
      ISSN = {0920-3036},
   %  CODEN = {KTHEEO},
  % MRCLASS = {19K35 (46L85 58J22)},
 % MRNUMBER = {1703305 (2000g:19004)},
%MRREVIEWER = {Hiroshi Takai},
       DOI = {\href{http://dx.doi.org/10.1023/A:1007744304422}{10.1023/A:1007744304422}},
}

\bib{Vie}{thesis}{
	AUTHOR = {Vieira, Felipe},
	TITLE  = {C*-algebras associated with endomorphisms of groups},
	SCHOOL = {University of M\"unster},
	YEAR   = {2013},
	NOTE    = {summary available as \href{http://arxiv.org/pdf/1308.1386v2}{arxiv:1308.1386v2}},
}

\bib{Wal}{book}{%MR648108,
    AUTHOR = {Walters, Peter},
     TITLE = {An Introduction to Ergodic Theory},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {79},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {New York},
      YEAR = {1982},
     PAGES = {ix+250},
      ISBN = {0-387-90599-5},
   %MRCLASS = {28Dxx (54H20 58F11)},
  %MRNUMBER = {648108 (84e:28017)},
%MRREVIEWER = {M. A. Akcoglu},
}

\bib{Wat}{article}{%MR996807,
    AUTHOR = {Watatani, Yasuo},
     TITLE = {Index for C*-subalgebras},
   JOURNAL = {Mem. Amer. Math. Soc.},
 % FJOURNAL = {Memoirs of the American Mathematical Society},
    VOLUME = {83},
      YEAR = {1990},
    NUMBER = {424},
     PAGES = {vi+117},
      ISSN = {0065-9266},
   %  CODEN = {MAMCAU},
%   MRCLASS = {46L05 (19K14 46L40 46L80 46M20)},
 % MRNUMBER = {996807 (90i:46104)},
%MRREVIEWER = {Masatoshi Enomoto},
       DOI = {\href{http://dx.doi.org/10.1090/memo/0424}{10.1090/memo/0424}},
}

\bib{Wil}{book}{%MR2288954,
    AUTHOR = {Williams, Dana P.},
     TITLE = {Crossed Products of C*-Algebras},
    SERIES = {Mathematical Surveys and Monographs},
    VOLUME = {134},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {2007},
     PAGES = {xvi+528},
      ISBN = {978-0-8218-4242-3; 0-8218-4242-0},
  % MRCLASS = {46-02 (22D25 46L05 46L35 46L55 46L85)},
 % MRNUMBER = {2288954 (2007m:46003)},
%MRREVIEWER = {Jonathan M. Rosenberg},
}

\bib{Wil2}{thesis} {%MR2941447,
    AUTHOR = {Willis, Paulette Nicole},
     TITLE = {C*-Algebras of labeled graphs and $*$-commuting endomorphisms},
      NOTE = {Thesis (Ph.D.)--The University of Iowa},
 PUBLISHER = {ProQuest LLC, Ann Arbor, MI},
      YEAR = {2010},
     PAGES = {113},
      ISBN = {978-1124-07016-2},
  % MRCLASS = {Thesis},
 % MRNUMBER = {2941447},
}

\bib{Win}{article}{%MR2179780,
    AUTHOR = {Winter, Wilhelm},
     TITLE = {On topologically finite-dimensional simple C*-algebras},
   JOURNAL = {Math. Ann.},
 % FJOURNAL = {Mathematische Annalen},
    VOLUME = {332},
      YEAR = {2005},
    NUMBER = {4},
     PAGES = {843--878},
      ISSN = {0025-5831},
   %  CODEN = {MAANA},
  % MRCLASS = {46L85 (19K14 46L05 46L35)},
 % MRNUMBER = {2179780 (2006i:46102)},
%MRREVIEWER = {Huaxin Lin},
       DOI = {\href{http://dx.doi.org/10.1007/s00208-005-0657-z}{10.1007/s00208-005-0657-z}},
}

\bib{Yee}{article} {%MR2301938,
    AUTHOR = {Yeend, Trent},
     TITLE = {Groupoid models for the C*-algebras of topological higher-rank graphs},
   JOURNAL = {J. Operator Theory},
  %FJOURNAL = {Journal of Operator Theory},
    VOLUME = {57},
      YEAR = {2007},
    NUMBER = {1},
     PAGES = {95--120},
      ISSN = {0379-4024},
  % MRCLASS = {46L05 (22D25 46L55)},
 % MRNUMBER = {2301938 (2008f:46074)},
}

\bib{Zel}{article} {%MR0241994,
    AUTHOR = {Zeller-Meier, Georges},
     TITLE = {Produits crois\'{e}s d'une C*-alg\`{e}bre par un groupe d'automorphismes},
   JOURNAL = {J. Math. Pures Appl. (9)},
%  FJOURNAL = {Journal de Math\'ematiques Pures et Appliqu\'ees. Neuvi\`eme
 %             S\'erie},
    VOLUME = {47},
      YEAR = {1968},
     PAGES = {101--239},
      ISSN = {0021-7824},
%   MRCLASS = {46.65},
%  MRNUMBER = {0241994 (39 \#3329)},
%MRREVIEWER = {B. Russo},
}

\end{biblist}
%\end{bibdiv} 
